Evaluating LLMs on Entity Disambiguation in Tables

Tables are crucial containers of information, but understanding their meaning may be challenging. Over the years, there has been a surge in interest in data-driven approaches based on deep learning that have increasingly been combined with heuristic-based ones. In the last period, the advent of \acf{llms} has led to a new category of approaches for table annotation. However, these approaches have not been consistently evaluated on a common ground, making evaluation and comparison difficult. This work proposes an extensive evaluation of four STI SOTA approaches: Alligator (formerly s-elbat), Dagobah, TURL, and TableLlama; the first two belong to the family of heuristic-based algorithms, while the others are respectively encoder-only and decoder-only Large Language Models (LLMs). We also include in the evaluation both GPT-4o and GPT-4o-mini, since they excel in various public benchmarks. The primary objective is to measure the ability of these approaches to solve the entity disambiguation task with respect to both the performance achieved on a common-ground evaluation setting and the computational and cost requirements involved, with the ultimate aim of charting new research paths in the field.

==> old_sections/old-01-intro.tex <==
\textbf{Tables} are commonly used to create, organise, and share information and play a crucial role across various business and science sectors. With the rise of the Open Data movement, tables are becoming more popular as a format for presenting information on the web. This has led to the publication of many online tabular data sources covering various domains such as finance, mobility, tourism, sports, and cultural heritage~\cite{Neumaier2016}. However, even with headers, understanding the meaning of tabular data can be challenging. As a result, there has been an increased focus on table interpretation (or \acl{sti}) in recent years.

One key element that supports such a process is \textbf{\ac{kgs}}.~\ac{kgs} are used to represent relationships between different entities such as people (\eg~Tom Hanks), places (\eg~Rome), mountains (\eg~Mont Blanc), events (\eg~Pitchfork Festival), and so forth~\cite{Hogan2021}. They arrange knowledge into graph structures, embedding the meaning of the data within the graph alongside the data itself. ~\ac{rdf}\footnote{\href{https://www.w3.org/RDF/}{www.w3.org/RDF/}} serves as a data model for representing \ac{kgs}, accompanied by a suite of languages and protocols designed to promote interoperable data management. In \ac{rdf}, graph nodes represent \textit{entities}, identified by URIs, or \textit{literals} (\eg~strings, numbers); edges represent \textit{relations} between entities or between entities and literals, which are identified by \ac{rdf} \textit{properties}. Entities and literals are associated with types (classes, \eg~\texttt{dbo:City} or datatypes, \eg~\texttt{xmls:integer}). The ontologies organise the possible types and properties and specify their meaning with logical axioms.

When information is available in unstructured or semi-structured formats, \eg tables or texts, \textit{finding links} between strings (or mentions) present in these sources and the entities they reference in a background \ac{kgs} becomes a key step of \textbf{\ac{sti}}. This aspect enables the integration, enrichment and extension of both the data and/or \ac{kgs}. We name this task \textbf{\ac{el}}, which comes in different flavours depending on the considered data formats but with some shared features.
For example, because of the ample entity search space, most of the approaches to \ac{el} include a first step where candidate entities for the input string are collected, \ie \textbf{\ac{er}}~\cite{Ratinov2009}, and a second step where the string is disambiguated by eventually selecting one or none of the candidate entities, \ie \textbf{\ac{ed}}~\cite{Rao2013}. In most approaches, \ac{er} returns a ranked list of candidates, while disambiguation consists of re-ranking the input list. Entity Disambiguation is at the heart of \ac{el}, with different approaches that leverage different kinds of evidence depending on the format and features of the input text~\cite{Shen2015}.

The interpretation of tables, also known as \ac{sti}, has gained much attention in different research communities, such as Semantic Web, Data Management, \ac{ai}, and \ac{nlp}. The increasing interest is exemplified by the international Semantic Web Challenge on Tabular Data to Knowledge Graph Matching (SemTab), proposed in 2019. In 2024, the challenge reached its fifth edition, and hand-crafted rules or heuristic-based approaches have mostly dominated Semtab's past editions.

\textcolor{blue}{
The advent of \textbf{\textit{\ac{llms}}} has led to a new category of approaches for table annotation. Based on the architecture structure of \ac{llms}, these approaches can be categorised into three groups: i) encoder-decoder \ac{llms}, ii) encoder-only \ac{llms}, and iii) decoder-only \ac{llms}~\cite{Pan2024}. Indeed, shortly after the first edition of SemTab, some works~\cite{Li2020,Deng2022,Suhara2022} applied encoder-only \ac{llms} to table interpretation. Although they did not participate in or compare with the SemTab challenge, they created a different experimental setting. 
During the SemTab2022 instead, a BERT-based~\cite{Devlin2019} model was combined with a more traditional approach~\cite{Huynh2022}. 
More recently, after the release of GPT-3.5~\cite{Ouyang2022} and open-source decoder-only \ac{llms} such as LLAMA~\cite{Touvron2023} and LLAMA 2~\cite{Touvron2023-2}, some works have begun applying encoder-based \ac{llms} to table interpretation~\cite{Li2023,Zhang2023}. In SemTab2023, a new decoder-only model was presented that uses BERT~\cite{Dasoulas2023}.
}

Our work starts from an observation: latest approaches for \textbf{\textit{LLM-based table understanding and manipulation} (LLM-TUM)} are evaluated in experimental settings which do not consider SemTab data in their evaluation; on the contrary, most of the \ac{sti} approaches evaluated on SemTab data do not consider data used to evaluate LLM-TUM approaches. In particular, we focus on \ac{el} in tables (CEA, in the \ac{sti} terminology), which is relevant not only to support table understanding but also to support data enrichment and integration pipelines, which are particularly interesting for the data management and Semantic Web community. The research objective of this paper is to shed more light on how different families of approaches developed for LLM-TUM or \ac{sti} compare on this task, considering more robust evaluation settings than the one available in papers published today. While doing so, we address some limitations of the experiments shared in some related works, \eg by providing more realistic settings for \ac{er}.  
As a result, we remark that the objective of this paper is to evaluate existing models in more comprehensive settings that are representative of different approaches rather than introducing a new approach. 

\textcolor{blue}{
In detail, we provide an extensive evaluation between the \ac{sota} approaches in the three categories: \dagobah~\cite{Huynh2022} and \alligator (formally \selbat)~\cite{Avogadro2023}, for hand-crafted rules and heuristic-based approaches, \turl~\cite{Deng2022} for the encoder-only \ac{llm} approaches, and \tablellama~\cite{Zhang2023} for decoder-only \ac{llm}.
Among the many \ac{sti} approaches in \ac{sota}, the choice fell on these four for various reasons. 
DAGOBAH~\cite{Huynh2022} achieved high accuracy scores in SemTab 2020, 2021 and 2022 editions. Other systems that achieved high accuracy scores, like Mtab~\cite{Nguyen2021}, were also considered during the selection. Unfortunately, Mtab is no longer available. The other approaches, \alligator, \turl and \tablellama, were not initially developed within the framework of the SemTab challenge, but they can be considered state of the art.
}

As stated, to create an experimental setting that is as balanced as possible, only the phase \ac{ed} on tables (or \ac{cea}) will be taken into consideration. The \ac{er} functionality will be provided by \lamapi (\textit{La}bel \textit{m}atching \textit{API})~\cite{Avogadro2022}, a comprehensive tool for IR-based \ac{er}, augmented with type-based filtering features. The tool facilitates string-based retrieval, a process involving searching and extracting information from a dataset by matching strings of characters. When queries are submitted, the retrieval task entails identifying relevant entities that match the given query or criteria. The choice to use \lamapi as an \ac{er} system is based on its demonstrated excellent results compared to other systems (\eg Wikidata Lookup). Additional information on \lamapi is available in the Section~\ref{sec:tested-approaches}.

\textcolor{blue}{
The ultimate aim is to shed light on the real capabilities of generative models to produce semantic annotations, highlighting the pros and cons compared to ``classic'' heuristic-based models, also carrying out an analysis of the degree of ability of these approaches to address the key challenges of the \ac{sti}.}

This paper is organised as follows:
Section \ref{sec:sti-definition} formally defines the \ac{sti} process and summarises the challenges. Section~\ref{sec:sota} proposes a detailed examination of the techniques used by \ac{sti} approaches in the \ac{sota}. Section~\ref{sec:dataset} describes the datasets used to evaluate the selected approaches, which have been described in Section \ref{sec:tested-approaches}. Section~\ref{sec:evaluation} introduces the configuration parameters and the evaluation results. Eventually, we conclude this paper and discuss the future direction in Section~\ref{sec:conclusions}.
